Bayesian estimation for collisional thermometry and time-optimal holonomic quantum computation

In this thesis we deal with two different topics. In the first half we investigate how the Bayesian formalism can be introduced into the problem of quantum thermometry -- a field which exploits the high level of control in coherent devices to offer enhanced precision for temperature estimation. In particular, we investigate concrete estimation strategies, with focus on collisional thermometry, a protocol where a series of ancillae are sent sequentially to probe the system's temperature. We put forth a complete framework for analyzing collisional thermometry using Bayesian inference. The approach is easily implementable and experimentally friendly. Moreover, it is guaranteed to always saturate the Cram\'er-Rao bound in the long-time limit. Subtleties concerning the prior information about the system's temperature are also discussed and analyzed in terms of a modified Cram\'er-Rao bound associated with Van Trees and Sch\"utzenberger. Meanwhile, in the last part of the thesis we approach the problem of non-adiabatic holonomic computation. Namely, we investigate the implementation based on $\Lambda$-systems. It is known that a three-level system can be used in a $\Lambda$-type configuration in order to construct a universal set of quantum gates through the use of non-Abelian nonadiabatic geometrical phases. Such construction allows for high-speed operation times which diminish the effects of decoherence. This might be, however, accompanied by a breakdown of the validity of the rotating-wave approximation (RWA) due to the comparable timescale between counter-rotating terms and the pulse length, which greatly affects the dynamics. Here, we investigate the trade-off between dissipative effects and the RWA validity, obtaining the optimal regime for the operation of the holonomic quantum gates.

==> chapters/vonMises.tex <==
\cite{Cam1986, Vaart1998, Butler2007}. Since the Bayesian update rule is often accompanied by unwieldy integration factors used in the normalization, this method proves to be quite useful for asymptotic limits. The motivation is to find a suitable approximation for integrals of the type:

\begin{equation}
\mathcal{N} = \int_a^b e^{n f(x)}dx 
\end{equation}

For our purposes, we will consider approximation in the asymptotic limit where $n$ is large. The net effect is that for large enough $n$ the distribution will be peaked around the global minimum $x_0$ of $f(x)$. We can Taylor expand this function up to second order

\begin{equation}
f(x) = f(x_0) + \frac{f''(x_0)}{2}(x-x_0)^2 + O(x^3)    
\end{equation}

This means that we can express the integral as:

\begin{equation}
\mathcal{N} \approx e^{n f(x_0)} \int_a^b e^{-|f''(x_0)|\frac{(x-x_0)^2}{2}}dx 
\end{equation}

Here we write $f''(x_0) = -|f''(x_0)|$, given that $f''(x_0)$ is negative by hypothesis (the function must exhibit a global minimum, to behave like a proper distribution). Since $n$ is large we can take the limits of integration to infinity, since the distribution decays very fast when far away from the peak. This means that the approximate integral is Gaussian, and we can arrive at the desired result \cite{butler_2007}:


The Laplace's method can be used to approximate integrals of exponentials of the type:

\begin{equation}
\mathcal{N} = \int_a^b e^{n f(x)}dx \approx \sqrt{\frac{2 \pi}{n f''(x_0)}} e^{n f(x_0)}     
\end{equation}


Thus, the core idea of this technique is that we approximate well-behaved functions with a single peak with a normal integral, the price we pay, however, is that we have to maximize the function $f(x)$, a problem which is less complex, in general. It's also worth noting that the accuracy of approximation depends mainly on two factors: i) how sharply peaked the distribution is, and this. In most scenario this usually depends on how large $n$ is, since other parameters are fixed. And also ii) on the basis, or variable of integration, choice. In general the normalization constant depends on the chosen basis, and this can yield better or worse accuracy \cite{mackay_2019}, this means we can expect distributions closer to the normal distribution to be more accurate.

Finally, it can be shown \cite{tierney_1986} that further expansions yield terms of order:

\begin{equation}
\mathcal{N} \approx \sqrt{\frac{2 \pi}{n f''(x_0)}} e^{n f(x_0)} \left[ 1 + O(n^{-1}) \right]    
\end{equation}

To see this, we can Taylor-expand $f(x)$ up to third order and then introduce a new variable $y$ through the substitution:

\begin{equation}
y^2 \equiv \frac{(x - x_0)^2}{n \sigma^2}
\end{equation}

with $\sigma^2 \equiv 1/f''(x_0)$. This means that the approximation will be proportional to:

\begin{equation}
\int 
\exp\{-\frac{y^2}{2\sigma}\}
\exp\left\{
-\left[
f^{(3)}(x_0) \frac{\sigma^3 y^3}{3!}  +
f^{(4)}(x_0) \frac{\sigma^4 y^4}{4!}  
+...
\right]
\right\}
dy
\end{equation}

Now, we simply expand the second exponential with $e^{-x} \approx 1 - x + \frac{1}{2}x^2$, with respect to the term in the second exponential. The integral above will reduce to the calculation of the momenta of the normal distribution, since the exponential will multiply integer powers of $y$:

\begin{equation}
1 + \frac{1}{n} \left\{ 
-
\sigma^4 f^{(4)}(x_0) \frac{\avg{y^3}{}}{24}
+
\sigma^6 f^{(3)}(x_0)^2 \frac{\avg{y^4}{}}{72}
\right\} + ...   
\end{equation}

Several terms were suppressed since the momenta of odd-power vanish for the normal distribution. Thus, as we can see, the leading order terms will be of order $O(n^{-1})$ after a more careful consideration.
